Learning Multi-Modal Nonlinear Embeddings: Performance Bounds and an Algorithm

While many approaches exist in the literature to learn low-dimensional representations for data collections in multiple modalities, the generalizability of multi-modal nonlinear embeddings to previously unseen data is a rather overlooked subject. In this work, we first present a theoretical analysis of learning multi-modal nonlinear embeddings in a supervised setting. Our performance bounds indicate that for successful generalization in multi-modal classification and retrieval problems, the regularity of the interpolation functions extending the embedding to the whole data space is as important as the between-class separation and cross-modal alignment criteria. We then propose a multi-modal nonlinear representation learning algorithm that is motivated by these theoretical findings, where the embeddings of the training samples are optimized jointly with the Lipschitz regularity of the interpolators. Experimental comparison to recent multi-modal and single-modal learning algorithms suggests that the proposed method yields promising performance in multi-modal image classification and cross-modal image-text retrieval applications.

==> sections/2RelatedWork_old.tex <==
\section{RELATED WORK}
\label{sec:RelatedWork}


The multi-modal learning approaches in the literature can be mainly grouped as co-training methods, multiple kernel learning algorithms, subspace learning approaches and deep learning methods. Co-training methods learn separate models in different modalities by encouraging their predictions to be similar \cite{BlumM98}. The study in \cite{coTrainingEM} improves the co-training algorithm using Expectation Maximization (EM) to assign probabilistic labels to unlabeled samples, where each modality classifier iteratively uses the probabilities of class labels. A probabilistic model for Support Vector Machine (SVM) is constructed in \cite{coEM} based on the Co-EM approach. There also exist co-regression algorithms employing the co-training idea. A regression algorithm that uses two k-NN regressors is presented to learn appropriate labels for unlabeled samples in \cite{coRegularization}. The co-training technique is also used in graph-based methods such as \cite{bayesianCoTraining}, where a Gaussian process model is used on an undirected Bayesian graph representation for all modalities. Co-training algorithms have been applied to multi-modal data analysis in various applications \cite{fusionCotraining}, \cite{multimodalVideoCotraining}, \cite{DuanTTLH17}.


%erased: \cite{multimodalWebCotraining}

% To add: \cite{multiViewImageClassification}. TIP 2020
%The existence of extra training samples may improve the classification and retrieval performance of multi-modal learning algorithms. The consensus of the cross-modal data reduces the disagreement between modalities \cite{surveyMultiviewLearning}, \cite{multiViewImageClassification}. Additional useful information in other modalities increases learning accuracy \cite{surveyMultiviewLearning}. Therefore, multi-modal learning algorithms have advantages than single-modal learning algorithms. In the literature, multi-modal learning approaches are grouped as co-training technique, multiple kernel learning algorithms, subspace learning-based approaches and deep learning methods. 


Subspace learning methods are based on computing linear projections or transformations that suitably align samples from different modalities. The well-known unsupervised subspace learning algorithm CCA (Canonical Correlation Analysis) maximizes the correlation between different modalities \cite{surveyOnMl}. Alternative versions of CCA such as cluster CCA \cite{clusterCCA}, multi-label CCA \cite{multilabelCca} and three-view CCA \cite{threeViewCca} have been proposed to improve the performance of CCA in various supervised tasks, all of which employ linear projections. In the recent years, many supervised subspace methods have been proposed, which aim to enhance the between-class separation and cross-modal alignment when learning linear projections of data. \revis{The GMLDA (Generalized Multiview Analysis) method proposes a multi-modal extension of the LDA algorithm within this framework \cite{gma}. Projection directions for different modalities are learnt by optimizing a quadratic objective function that contains within-class scatter, between-class scatter, and cross-modal correlation terms \cite{gma}. A kernel extension of the GMLDA algorithm for learning nonlinear mappings is also presented in \cite{gma}. Following the approach in  \cite{gma}, many extensions of this work have been proposed in succeeding studies. In  \cite{KanSZLC16}, a view consistency term is added to the objective function of GMLDA so as to impose the similarity of the linear projection functions of different views. The cross-media retrieval method in \cite{WeiZZWXFY16} addresses a supervised linear projection learning problem as in \cite{gma}; however, applies regularization on projection matrices. Several works have focused on kernel extensions of the problem \cite{JingHZWLY14}, \cite{CaoICG18}. The KMvMDA (Kernel Multi-View Modular Discriminant Analysis) method proposed in \cite{CaoICG18} learns kernel representations by imposing within-class and between-class correlation constraints across different modalities. The kernel method in \cite{SunXY16} uncorrelates the feature vectors of the individual modalities as an additional consideration. Another body of methods model data by constructing label-aware data graphs and 
include a graph-based regularization term in the objective in order to preserve the geometry of the data set \cite{YinWW17},  \cite{ZhangMLHT18}. The JFSSL (Joint Feature Selection and Subspace Learning)  method uses a joint graphical model for calculating projections with relevant and irrelevant features \cite{jfssl}.}  Various methods are based on combining kernels in different modalities, such as convex combinations of multiple Laplacian kernels \cite{ArgyriouHP05}, or the power mean of multilayer graph kernels \cite{MercadoTH19}. \revis{Among all these methods, our method bears similarities to especially supervised kernel methods in that it learns  nonlinear data representations in view of class separation and cross-modality alignment objectives. On the other hand, it has two major differences from these approaches: (1) Our nonlinear representation model is particularly flexible and effective as the pointwise embeddings of training samples are optimized individually by respecting the data geometry. (2) We explicitly incorporate the generalization performance of the algorithm in the objective function, which is a unique and distinctive feature of our method.} While there are multi-view algorithms learning pointwise nonlinear mappings as in our method, these often address unsupervised problems such as spectral embedding \cite{spectralEmbeddingMv} and multi-modal clustering \cite{multimodalJointClustering}.










%
%Ext 9,10: Subspace methods (Skip)
%Ext2: Skip for now (similarities expressed in a different way)
%Ext3: (Fei Wu et al, Slightly related, may skip ) Adapts the idea to the cross-media ranking problem, where the projection directions are optimized so as to adjust the cross-modality correlation term by weighing the sample pair alignment terms with respect to their  relative ranking positions. 
%Ext7: Skip, ranking method like Ext3
% Some subspace learning methods propose solutions based on the metric learning \cite{metricLearning} and matrix factorization \cite{matrixFactorization} ideas.






In the recent years, deep learning methods have provided quite effective solutions for analyzing large multi-modal data sets. Deep multi-view autoencoders can learn shared representations  \cite{multimodalDeepLearning}, \cite{FengWL14}, \cite{mmRetrievalDeepLearning}, or cross-weights  \cite{deepMultimodalCrossWeights} across different data modalities. Convolutional neural networks are widely used in multi-modal problems as well, where CNN structures for visual modalities can be combined with other modalities at the feature level \cite{WeiZLWLZY17}, \cite{CastrejonAVPT16}, \cite{multimodalDeepImageAnnotation}, or the classifier level \cite{multiViewImageClassification}. GAN-type architectures adversarially train feature generators and domain discriminators across different modalities \cite{deepMultimodalRepresentation}. The method in \cite{ZhaoDF17} learns a common latent representation for different modalities via a deep matrix factorization scheme. 


\revis{Some previous studies proposing a theoretical analysis of multi-view learning are the following. The study in \cite{BlumM98} analyses the learnability of joint models in the two-view co-training problem, assuming the conditional independence of two views. Several other PAC-style bounds are proposed in \cite{DasguptaLM01}, \cite{SunSM17}, mainly stating that the agreement of the classifiers of the two views on training data guarantees a good estimate of the expected test error. Several studies have proposed generalization bounds for co-regularized RKHS methods \cite{RosenbergB07}, \cite{Sun11}, \cite{XuTX15} in terms of the Rademacher complexities of the involved function classes. These previous analyses differ from ours in that they all aim to bound the difference between the training loss and the expected loss in multi-view classification, while our analysis addresses the particular problem of nonlinear dimensionality reduction in multi-modal learning. Our distinctive contribution is that we explicitly characterize the geometric properties and the regularity conditions of the nonlinear embedding to achieve successful generalization.}

%The performance of the SVM-2K algorithm combining the KCCA and SVM approaches is analyzed in \cite{FarquharHMSS05}. 

Finally, some other previous works related to our study are the following. The theoretical analysis in  \cite{supervisedManifold} provides performance bounds for supervised nonlinear embeddings in a single modality. The idea in \cite{supervisedManifold} is developed in this paper to perform a theoretical analysis for multi-modal embeddings. The previous work \cite{nsse} proposes a supervised nonlinear dimensionality reduction algorithm via smooth representations like in our work; however, it treats the embedding problem in a single modality. Lastly, a preliminary version of our work was presented in \cite{KayaV19}. The current paper builds on \cite{KayaV19} by including a theoretical analysis of the multi-modal learning problem and significantly extending the experimental results. 




==> sections/8Biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

%
%
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/semihPhoto.jpg}}]{Semih Kaya}
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%\end{IEEEbiography}
%
%% if you will not have a photo at all:
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/semihPhoto.jpg}}]{Elif Vural}
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%Biography text here.
%\end{IEEEbiography}
